UniSumm and SummZoo: Unified Model and Diverse Benchmark for Few-Shot Summarization

The high annotation costs and diverse demands of various summarization tasks motivate the development of few-shot summarization. However, despite the emergence of many summarization tasks and datasets, the current training paradigm for few-shot summarization systems ignores potentially shareable knowledge in heterogeneous datasets. To this end, we propose \textsc{UniSumm}, a unified few-shot summarization model pre-trained with multiple summarization tasks and can be prefix-tuned to excel at any few-shot summarization task. Meanwhile, to better evaluate few-shot summarizers, under the principles of diversity and robustness, we assemble and release a new benchmark \textsc{SummZoo}. It consists of $8$ summarization tasks with multiple sets of few-shot samples for each task, covering diverse domains. Experimental results and analysis show that \textsc{UniSumm} outperforms strong baselines by a large margin across all sub-tasks in \textsc{SummZoo} under both automatic and human evaluations and achieves comparable results in human evaluation compared with a GPT-3.5 model.

==> case1.tex <==
\begin{table*}[h]
\renewcommand{\arraystretch}{1.5}
    \centering
    \small
    \begin{tabular}{l|p{13.5cm}}
    \thickhline
    \multicolumn{2}{c}{\textbf{MultiNews}}\\
    \thickhline
        Input text  & paris (ap)  the pompidou centre in paris hopes to display a long-vanished picasso painting in may, now that it has been recovered by u.s. customs authorities. this undated photo provided by the united states department of justice, shows a cubist painting entitled the hairdresserby pablo picasso. authorities say the painting worth millions of dollars was ... ||||| a stolen picasso worth millions of dollars was shipped to the u.s. in a package that described it as a \$37  "art craft "  but it will soon be on its way back to france...    \\
        \hline
        PEGASUS & – a 1911 cubist painting worth millions of dollars has been recovered after being mysteriously transported from france to the us nearly a decade ago. the pablo picasso painting, titled la coiffeuse, was reported missing from a pompidou storeroom in paris in 2001 \underline{and was last seen in a package shipped to the us from belgium}, the ap reports. federal prosecutors in brooklyn filed papers thursday to seize the painting, which was hidden in a climate-controlled storage facility in queens, ny, and will soon be returned to france, reports the new york times. the center for art recovery in paris says it hopes to have the painting back in may, at a time when the cultural world is reeling from islamic state videos showing the destruction of statues in iraq. "this is a true comfort for us at a time when the cultural world is reeling from the islamic state video showing the destruction of statues in iraq," says alain seban, the director of the pompidou centre in paris. "it is a work of art that represents the genius of pablo picasso and was bequeathed to us in 2001 by the master of france's national museum."\\
        \hline
        {\makecell[l]{\textsc{UniSumm}}} & - a century-old picasso painting missing from paris for more than a decade resurfaced in the united states under false pretenses as a \$37 holiday-themed "art craft," the ap reports. the 1911 painting, called "la coiffeuse," \underline{was unearthed in december in a fedex shipment from belgium to newark}. the canvas had been smuggled out of a storeroom of the centre georges pompidou, the paris museum and arts center. officials there thought it was safe and sound until they received a loan request for it in 2001. they searched the storerooms and could not find it. on dec. 17, someone going by "robert" with an address in belgium brought the painting to a climate-controlled warehouse in long island city and was seized, the ap reports. the us attorney for the eastern district of new york filed a civil complaint thursday to forfeit the picasso and return it to france. the canvas, titled "la coiffeuse," was bequeathed to the national museums of france in 1998. the pompidou director alain seban said in a statement friday that he hopes the work can be exhibited again publicly in may. no arrests have been made in the case.  \\
        \hline
        {Gold} & - a picasso painting that was found to have vanished from a paris museum more than a decade ago has \underline{turned up 2014 in the us, in a package shipped from belgium.} its papers identified it as a \$37 "art craft/toy" and also included the line "joyeux noel," or merry christmas, the new york times reports. a man named "robert" attempted to send the package to a climate-controlled warehouse in queens, new york, in december, but custom officials at the port of newark seized what turned out to be picasso's 1911 la coiffeuse (the hairdresser). french museum officials traveled to new york last month and confirmed the find is indeed the missing picasso work, which the centre georges pompidou realized was missing from its storerooms in 2001 following a loan request; it was then valued at more than \$2.5 million. court documents don't specify whether the sender or would-be recipient have been identified, nbc news reports, but "a lost treasure has been found," us attorney loretta lynch said in a statement. she filed a civil complaint yesterday that will have the painting returned to france. the pompidou's director, who called the painting's rediscovery a "true comfort," hopes the painting can go on display at the museum as early as may, the ap reports. (another picasso work was stolen days before this one was found.) \\
    \thickhline
    \end{tabular}
    \caption{Case study (b): Gold and generated summaries by 100-shot PEGASUS and \textsc{UniSumm} on MultiNews, respectively.
    ``|||||'' seperates different reports in the input. }
    \label{tab:case_multinews}
\end{table*}
